Graph Neural Networks for Tabular Data Learning: A Survey with Taxonomy and Directions

In this survey, we dive into Tabular Data Learning (TDL) using Graph Neural Networks (GNNs), a domain where deep learning-based approaches have increasingly shown superior performance in both classification and regression tasks compared to traditional methods. The survey highlights a critical gap in deep neural TDL methods: the underrepresentation of latent correlations among data instances and feature values. GNNs, with their innate capability to model intricate relationships and interactions between diverse elements of tabular data, have garnered significant interest and application across various TDL domains. Our survey provides a systematic review of the methods involved in designing and implementing GNNs for TDL (GNN4TDL). It encompasses a detailed investigation into the foundational aspects and an overview of GNN-based TDL methods, offering insights into their evolving landscape. We present a comprehensive taxonomy focused on constructing graph structures and representation learning within GNN-based TDL methods. In addition, the survey examines various training plans, emphasizing the integration of auxiliary tasks to enhance the effectiveness of instance representations. A critical part of our discussion is dedicated to the practical application of GNNs across a spectrum of GNN4TDL scenarios, demonstrating their versatility and impact. Lastly, we discuss the limitations and propose future research directions, aiming to spur advancements in GNN4TDL. This survey serves as a resource for researchers and practitioners, offering a thorough understanding of GNNs' role in revolutionizing TDL and pointing towards future innovations in this promising area.

==> 5-Applications.tex <==
\section{Applications}
\label{sec-app}
TBA
\ct{describe TDL applications in which GNN outperforms existing tabular data learning methods}

\subsection{Anomaly Detection}
\label{subsec-fraud}
Anomaly detection on tabular data is a crucial task in data analysis, aiming to identify data points or observations that deviate significantly from the normal behavior as represented by the majority of the data. These anomalies, also known as outliers, could indicate data entry errors, unexpected events, or crucial insights. Problematically, anomalies are rare and differ from the norm in complex and often unknown ways, making it difficult to provide a single, encompassing definition of what constitutes an anomaly. Current approaches in anomaly detection generally revolve around statistical, machine learning, and distance-based methods. Statistical methods rely on assuming a statistical model for normal behavior and flagging data points that do not fit this model. Machine learning techniques involve training a model (like a neural network, decision tree, or support vector machine) on normal data and then marking data points the model struggles to predict as anomalies. Distance-based methods identify outliers by considering the distance or similarity of a data point to its neighbors.

Existing approaches to tabular data anomaly detection have three main limitations, which can potentially be mitigated using GNNs. (1) \textit{Inability to capture complex dependencies}. Traditional statistical and distance-based methods typically make strong assumptions about the data distribution (e.g., Gaussian distribution), which may not always hold true. They often fail to capture complex dependencies between features, particularly for high-dimensional data. Moreover, most distance-based methods view each data point in isolation and evaluate its similarity with its closest neighbors, ignoring the broader context of the dataset. In contrast, GNNs effectively model the interactions between various features and consider the global structure of the data, providing a more nuanced detection of anomalies~\cite{lunar22,du2022graph,xiao2023graph}. (2) \textit{Insufficiency in dealing with relational data}: Traditional anomaly detection approaches do not inherently account for relational data or complex dependencies across instances, which could be crucial for identifying anomalies in certain contexts. GNNs are designed to handle relational data and can propagate information across nodes (features), capturing non-linear, complex interactions that could indicate anomalies~\cite{cfath21,h2fd22,ihgat21kdd,caregnn20}. (3) \textit{Difficulty in handling categorical data}: Traditional methods often struggle with categorical data, requiring additional preprocessing steps such as one-hot encoding. GNNs, by treating each category as a distinct node in the graph, can handle categorical data more naturally~\cite{zhang2022hierarchical,xfraud21,cfath21}. Below we review three main categories of studies that leverage GNNs for anomaly detection on tabular data. They are GNN-based unsupervised detection, fraud detection, and fault detection.

\textbf{GNN-based Unsupervised Detection.}
LUNAR~\cite{lunar22} enhances the adaptability and expressivity of traditional local outlier methods. By unifying local outlier methods within the message passing framework of GNNs, LUNAR learns to leverage information from neighboring nodes in a trainable manner to detect anomalies on tabular data.
By devising graph autoencoder (GAE)~\cite{du2022graph} to propagate feature values and alter the distribution pattern of the dataset, outliers that are embedded within normal regions or dense clusters can be accurately detected. GAE here involves converting the Euclidean structured data into a graph, training the GAE using both the dataset and its corresponding graph, and identifying outliers based on the objects that are difficult to reconstruct in the GAE's output layer.
A follow-up work further regularizes the graph autoencoder~\cite{gramst22} and incorporates a minimum spanning tree-based distance metric into the process of feature aggregation.


\textbf{GNN-based Fraud Detection.}
Anomaly detection and fraud detection are closely related as they both involve identifying irregular patterns or behaviors from tabular-like data. Fraud detection specifically uncovers fraudulent activities that involve deceit, manipulation, or illegal actions for financial gain. Real-world applications of fraud detection includes credit card fraud, review fraud, customs fraud, malicious account, and online transaction fraud. GNNs can be applied to fraud detection due to their ability to capture complex relationships and dependencies in data. In fraud detection, data often exhibits intricate connections, whose modeling is the strength of GNNs. GNN-based fraud detection has two main types, i.e., learning GNNs on homogeneous or heterogeneous graphs constructed from tabular data. The formulation of homogeneous graph involves creating edges to connect individuals who share common attributes~\cite{caregnn20,pcgnn21,h2fd22,aognn22} while that of heterogeneous graph establishs multi-typed relationships among entities that could be individuals and various attributes~\cite{ihgat21kdd,zhang2022hierarchical,cfath21,xfraud21}.
For homogeneous GNNs on fraud detection, CARE-GNN~\cite{caregnn20} learns to defend against camouflaged fraudsters through an adaptive neighor selection. PC-GNN~\cite{pcgnn21} deals with the label imbalance issue by devising a label-balanced neighbor sampler for GNNs. AO-GNN~\cite{aognn22} optimizes the AUC scores of fraud detection on GNNs. H2-FDetector~\cite{h2fd22} further develops different message passing mechanisms for homophilic and heterophilic connections in the graph. For heterogeneous GNNs on fraud detection, IHGAT~\cite{ihgat21kdd} utilizes the cross-interaction information over transactions and intentions to better learn the representations of individuals. xFraud~\cite{xfraud21} brings explainability into GNN-based fraud transaction detection. C-FATH~\cite{cfath21} copes with structure-inconsistency and content-inconsistency among individuals in fraud detection. HMF-GNN~\cite{zhang2022hierarchical} further encodes longitudinal and multi-modal knowledge during GNN learning. GraphFC~\cite{graphfc23} is a fraud detection method designed to tackle the challenges of label scarcity and unseen records in transaction tabular data. By constructing a heterogeneous graph that captures the relationships between transactions and their attributes, GraphFC enables self-supervised GNNs to effectively leverage limited supervision signals and exhibit inductive ability, enhancing its capability to detect customs fraud.

\textbf{GNN-based Fault Detection.}
Fault detection are closely related to anoamly detection as they both aim to identify deviations or abnormalities in tabular data. While anomaly detection is a broader concept that encompasses the detection of any unusual patterns, fault detection specifically focuses on identifying faults or failures in systems, such as mechanical equipment~\cite{sganm22,xiao2023graph} or industrial processes~\cite{iagnn21}, to ensure their proper functioning and prevent potential accidents or disruptions. IAGNN~\cite{iagnn21} represents the sensor tabular signals and their interactions as a graph, and utilizes multiple GNN blocks to extract fault features from subgraphs with different edge types. IAGNN can learn and integrate multiple interactions between sensor signals, enabling the extraction of fault features that incorporate both raw data information and implicit interactions, ultimately enhancing fault detection in complex industrial processes. 
SGANM~\cite{sganm22} recognizes new fault types in fault diagnosis models, even with limited labeled samples. By leveraging meta-learning and exploiting relationships among samples through constructing a spatial-temporal graph-based approach, SGANM enhances the meta-learner's ability to learn meta-knowledge and generalize to target fault diagnosis. 
By constructing a graph based on sample similarity and utilizing a GNN for feature mapping, GNNBFD~~\cite{xiao2023graph} incorporates neighbor information to enhance the fault detection task, enabling the identification of faulty samples with low degrees of failure.

\subsection{CTR Prediction}
\label{subsec-ctr}
Click-through rate (CTR) prediction on tabular data is a critical task in various online services like digital advertising, web search, and recommendation systems. The goal is to forecast whether a user will click on a presented item based on a multitude of features encoded in tabular forms, such as user demographics, past behavior, item attributes, and context variables. The problem is essentially a binary classification task, wherein the output indicates if a user will click (1) or not (0). Existing approaches for CTR prediction typically utilize machine learning models like logistic regression, decision trees, and more recently, deep learning-based models. These models aim to capture intricate relationships between features and click behavior. Logistic regression, while computationally efficient, often struggles with complex feature interactions. To handle these interactions, models like decision trees, gradient boosting machines (like XGBoost), and deep learning methods (like DeepFM~\cite{deepfm17}, Wide\&Deep~\cite{wnd16}, and GCN-int~\cite{gcnint21}) are capable of extracting high-order feature interactions, providing more accurate predictions. There is also another line of research for a sequential recommendation (SR). Converse to the conventional CTR task, SR entails providing a list of recommended items based on the chronological order of user-item interactions. Addressing this challenge, RetaGNN~\cite{retagnn21} introduces a novel approach that leverages a user-item-attribute tripartite graph in conjunction with the Rational Attentive Graph Neural Network (RA-GNN). This architecture enables RetaGNN to train a recommendation system with a holistic capability. In particular, it excels at predicting the subsequent items in diverse settings, including conventional, inductive, and transferable scenarios.
 

 The three most critical issues of existing approaches to CTR prediction can be properly handled by GNNs. (1) \textit{Sparse Data and Cold-start Problem}: Existing approaches often struggle with sparse data and cold-start issues. New users or items, which lack historical interaction data, are challenging for these models to handle. By leveraging the structural information of user-item interaction graphs, GNNs can alleviate this problem by propagating information from the connected nodes. GME~\cite{gme21} constructs a graph to connect old ads with new ones to improve the cold-start problem. (2) \textit{Complex Feature Interactions}: Existing methods sometimes fail to model complex feature interactions efficiently and effectively. By treating features as node attributes in the graph and learning to aggregate and transform these attributes, GNNs can inherently capture complex high-order feature interactions. Fi-GNN~\cite{fignn19} leverage GNN to model the interactions between features, whereas Cross-GCN~\cite{crossgcn21} introduces a novel technique called Cross-feature Graph Convolution, which enhances feature transformations by capturing the interactions between features. (3) \textit{User and Item Heterogeneity}: Users and items usually have multiple types or belong to multiple categories, making the user-item interactions heterogeneous. Existing methods might not handle this heterogeneity well. GNNs can accommodate this by using different types of nodes and edges in the graph to represent different types of users and items. DisenCTR~\cite{disenctr22} constructs
a time-evolving user-item interaction graph and utilizes the concept of disentangled representation learning to extract diverse user interests. DE-GNN~\cite{dgenn21} proposes dual graphs for solving feature sparsity (infrequent occurrence of many features) and user behavior sparsity (short behavior sequences exhibited by numerous users) issues. 






\subsection{Medical Prediction}
\label{subsec-med}
Medical prediction involves several major tasks, such as disease prediction~\cite{dpgnn21,wpn21,riognn22}, representation learning of patients, and Electronic Medical Records (EMRs)~\cite{riognn22,hsgnn20,ssgnet22,hcl22,medgraph20,gct20}, medication recommendation~\cite{gate20}, and survival prediction~\cite{lstmgnn21,riognn22,mgnn22}. In the context of medical prediction tasks, the input typically relies on EMRs, which provide comprehensive details about each patient visit, diagnostic codes, treatment information, and disease indicators. EMRs inherently capture diverse relationships, encompassing code-code associations, patient-patient connections, and patient-code correlations. 
he introduction of GNN helps improve the three limitations in medical prediction tasks. (1) \textit{Structural and Temporal Information}: Previous research on medical prediction without the usage of GNNs often ignores the intrinsic structure and temporal dynamics present in EMRs. By treating the codes within each EMR as nodes, one can effectively incorporate the structural information and capture the temporal effects through the application of GNNs. (2) \textit{Data sparsity}: Developing a prediction model that can effectively generalize to rare diseases poses a considerable challenge due to the sparsity of their medical records and the heavy reliance of model performance on data abundance. Nevertheless, GNNs offer a promising approach to address this issue by leveraging external knowledge and treating it as interconnected nodes. By aggregating information from neighboring nodes, GNNs facilitate the effective integration of external knowledge, thereby enhancing the model's ability to generalize and make accurate predictions for rare diseases. (3) \textit{EMR Heterogeneity}: EMRs encompass diverse patient information, visit details, diagnoses, and medications, forming a complex and heterogeneous graph-like structure. Consequently, the utilization of GNN becomes essential to effectively handle and exploit the intricacies inherent in this data structure.




\subsection{Missing Data Imputation}
\label{subsec-impute}
Missing data imputation refers to the task of replacing missing or null values in tabular datasets with substituted values. This task arises from the practical issue that datasets, especially in real-world scenarios, are often incomplete due to various reasons, such as data collection errors, privacy issues, or unexpected data corruption. The key idea of existing approaches to missing data imputation includes methods like mean or median imputation, regression imputation, and more sophisticated machine learning methods. There's also a growing trend towards using deep learning models, such as autoencoders~\cite{ginn20,egggae23}, for this task due to their ability to model complex relationships. The importance of missing data imputation spans across multiple domains, such as healthcare (e.g., filling missing medical records), finance (e.g., completing transactional data), environmental science (e.g., imputing missing climate data), and social sciences (e.g., filling gaps in survey data), as robust data sets with minimal missing values are crucial for precise and accurate predictive modeling.

Here we discuss three main shortcomings of existing approaches. (1) \textit{Non-random Missingness}: Conventional imputation methods often assume data is missing at random (MAR), which may not be the case in real scenarios. Graph structures can be leveraged to model dependencies that could give insights into the non-random nature of missingness, providing a more accurate imputation. GNN4MV~\cite{gnn4mv22} employs a direct classification approach for instances containing missing values by leveraging information from their neighbors. The construction of the graph in GNN4MV is guided by supervised signals, thereby mitigating the influence of missing values and ensuring the graph is constructed with more reliable proximity metrics. (2) \textit{Multivariate Missingness}: Traditional methods might falter when several variables have missing data, especially when these missing data patterns interrelate. By considering features as nodes in a graph and using GNNs, multivariate missingness can be addressed more effectively due to the ability of GNNs to capture inter-node (inter-feature) relationships. GEDI~\cite{gedi23} projects heterogeneous features into a common space and exploits the attention mechanism to capture the row-wise and column-wise interactions within the tabular data. GRIN~\cite{grin22} impute missing data by learning spatio-temporal representations of a multivariate time series through GNN.  (3) \textit{Less Correlation between Imputation and Target Prediction}: Existing learning-based methods, which either rely on non-missing features to infer the missing ones or utilize the distribution of feature values for imputation, cannot produce imputation outcomes that best benefit the target prediction. GRAPE~\cite{you2020grape} is a countermeasure by treating imputation as the edge weight prediction task and target prediction as the node label prediction task in an instance-feature bipartite graph, the influence of feature imputation on target labels can be considered. Similarly, IGRM~\cite{igrm23aaai} employs a friend network in the instance-feature bipartite graph to augment the ability to differentiate sample relationships.



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table*}[!t]
% \centering
% \caption{Summary of GNN4TDL applications. Column ``GNN Benefits'' briefly presents how GNNs benefit the application. Column ``Tabular Source'' gives where we can find the tabular data in the application. Column``GNN \textgreater ML'' indicates whether GNN-based models outperform which typical ML/DL models. }
% \label{tab:summary-app}
% % \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|l|l|l|l|l}
% \hline
%  & \multicolumn{1}{c|}{GNN Benefits} & \multicolumn{1}{c|}{Tasks} & \multicolumn{1}{c|}{Tabular Source} & \multicolumn{1}{c|}{GNN \textgreater ML} & \multicolumn{1}{c}{Key References} \\ \hline
% \multirow{3}{*}{Anomaly Detection} & \multirow{3}{*}{} & Unsupervised Detection &  &  &  \\ \cline{3-6} 
%  &  & Fraud Detection &  &  &  \\ \cline{3-6} 
%  &  & Fault Detection &  &  &  \\ \hline
% CTR Prediction &  & Binary Classification &  &  &  \\ \hline
% \multirow{5}{*}{Medical Prediction} & \multirow{5}{*}{} & Disease Prediction &  &  &  \\ \cline{3-6} 
%  &  & Patient Embedding &  &  &  \\ \cline{3-6} 
%  &  & EMR Modeling &  &  &  \\ \cline{3-6} 
%  &  & Medication Rec &  &  &  \\ \cline{3-6} 
%  &  & Survival Prediction &  &  &  \\ \hline
% \multirow{2}{*}{Missing Data Imputation} & \multirow{2}{*}{} & Static Imputation &  &  &  \\ \cline{3-6} 
%  &  & Temporal Imputation &  &  &  \\ \hline
% Modeling Relational DB &  & Label Prediction &  &  &  \\ \hline
% \end{tabular}%
% % }
% \end{table*}


\subsection{Financial Technology}
\label{subsec-fintech}
Financial technology, or FinTech, encompasses a broad array of technologies and applications designed to streamline, enhance, and digitize traditional financial systems and operations. In these contexts, tabular financial data -- structured data represented in tables such as transaction records, credit histories, customer databases, stock prices, etc. -- are integral for these applications' proper functioning. Applications using financial tabular data include asset price prediction~\cite{lifeprice23tkde,magnn22pr,rgsl22,tgc19tois}, risk management~\cite{yang2021financial,sgrn22ijcai}, investment decision-making~\cite{fingat21,kim2019hats}, fraud detection~\cite{xu2021towards}, credit scoring~\cite{amg20}, and personalized financial advice, among others. Problem tasks related to these applications often involve accurate prediction (e.g., credit default, stock market trends), anomaly detection (e.g., fraudulent transactions), or clustering for customer segmentation.

GNNs can be applied to financial applications with tabular data to provide a powerful tool for extracting complex patterns and relationships that are not immediately evident in tabular data alone. Traditional tabular data assumes independence between records, which is not always the case in the real world. Relationships, connections, or interactions between data entities could play crucial roles in many financial scenarios. Entities such as individuals, companies, stocks, and commodities are interconnected in various ways. A GNN can model these entities and their relationships in a graph structure, where nodes represent entities, and edges represent relationships between these entities. This can bring out hidden information in the data, providing more context and consequently better predictions.

GNNs offer a novel approach to stock prediction by recognizing and learning from the interconnections between different stocks, sectors, and broader market indicators. Traditional tabular data processing techniques treat each stock as an isolated unit, predominantly considering its past performance and maybe some fundamental features of the company. This often oversimplifies the complex and interconnected nature of the stock market. GNN-based approach provides an enriched context for prediction by incorporating how changes in one stock or a group of stocks may influence others. For example, a major price movement in a leading company's stock (e.g., Apple or Amazon) may affect related companies in the technology sector. 

In credit scoring, rather than treating each client independently, a GNN could model the connections between clients, such as shared transactions or common business relationships. This can provide additional information that is not evident in tabular data, such as how risk propagates through a network of borrowers.

Another area is in detecting financial fraud, which often involves coordinated activities among multiple accounts. Traditional tabular data-based approaches might treat each account's transactions independently, potentially missing suspicious patterns. However, by using GNNs, the interaction among different accounts can be better modeled, improving the ability to detect complex fraudulent activities.

GNNs are also useful for portfolio management and algorithmic trading. They can model and predict complex interactions between various financial instruments. They can help understand how the price of one stock might affect another or how a news event might impact a sector of stocks.

% In essence, GNNs offer an enriched perspective by leveraging the relational structure within financial data, which can significantly enhance the quality of decision-making and predictive analytics in finance.


% ~\cite{kim2019hats}
% ~\cite{tgc19tois}
% ~\cite{fingat21}
% ~\cite{rgsl22}
% ~\cite{sgrn22ijcai}
% ~\cite{xu2021towards}
% ~\cite{yang2021financial}
% ~\cite{magnn22pr}
% ~\cite{lifeprice23tkde}
% ~\cite{thgnn22cikm}
% ~\cite{li2023look}
% ~\cite{amg20}
% ~\cite{ami23tkde}

\subsection{Modeling Relational Databases}
\label{subsec-db}
GNNs provide a novel way to model relational databases by utilizing the inherent structure and relationships present in the data tables. GNNs propagate information across connections across data tables, thereby preserving richer relational context for data records. The inherent structure of database schema, consisting of multiple data tables, and the associations between entities and their attributes, are utilized as the base of graph construction. Nevertheless, existing studies of GNN applications in modeling relational databases are limited.

RDBToGraph~\cite{gnndb20} provide a novel approach to model relational databases by interpreting them as directed multigraphs. Each node in the graph corresponds to a row in the database, while the table, foreign key column, non-foreign key column, and foreign key reference correspond to node type, edge type, node feature, and directed edge, respectively. This approach allows the preservation of the relational structure inherent in the data, which often gets destroyed in the conventional ``flattening'' process for database handling. Flattening also involves arduous feature engineering, which GNNs bypass, offering a more efficient alternative. When predicting the label of a target row/node, a subgraph is selected from the full graph for GNN model training.

Siamese Graph Convolutional Networks (S-GCNs)~\cite{krivosheev2020siamese} provides the integration of structured and unstructured data sources such as relational databases and free text from news articles. The relational database is converted into a graph, where each record is a node, and the relations between records, which are inherent in the database, are represented as edges. Through tokenization and named entity recognition to identify entities and their relations from free text, the text graph can also constructed. These unstructured data graphs are linked to the structured database graph, allowing GNNs to learn a distance function between nodes for the task of record linkage.

A recent vision paper~\cite{vogel2022towards} presents the concept of relational representation learning which can utilize the full relational structure of databases, as opposed to focusing on single tables alone. The proposed model architecture combines language models (LMs) and GNNs to achieve this. LMs is to encode individual rows within tables, and GNNs is used to model both the relational structure within and across tables. This includes identifying rows that belong to the same table and understanding relationships between rows across different tables, based on the schema of the relational database. 

~\cite{gcfrd22cikm}
% By ~\cite{schema19acl}





==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tables/ablation_dp.tex <==
\begin{table*}[htbp]
    % \renewcommand{\arraystretch}{1.1}
    \caption{Performace gain (relative to the version of only using CLS embedding) with 3 different aggregations before feeding encoded representation into the downstream model.}
    \label{tab:ablation_dp}
    \centering
    \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.1\textwidth}|>{\centering\arraybackslash}p{0.1\textwidth}|>{\centering\arraybackslash}p{0.1\textwidth}}
    \hline
     & all & comp-all & cls \\
    \hline
    Concrete & \cellcolor{red!20}-7.27\% & \cellcolor{red!20}-10.55\% & \cellcolor{yellow!20}0.00\% \\
    Energy & \cellcolor{red!20}-2.24\% & \cellcolor{green!20}3.58\% & \cellcolor{yellow!20}0.00\% \\
    Housing & \cellcolor{green!20}7.27\% & \cellcolor{green!20}1.21\% & \cellcolor{yellow!20}0.00\% \\
    Kin8nm & \cellcolor{red!20}-6.78\% & \cellcolor{red!20}-7.93\% & \cellcolor{yellow!20}0.00\% \\
    Naval & \cellcolor{red!20}-139.86\% & \cellcolor{red!20}-53.79\% & \cellcolor{yellow!20}0.00\% \\
    Power & \cellcolor{green!20}1.98\% & \cellcolor{green!20}2.20\% & \cellcolor{yellow!20}0.00\% \\
    Wine & \cellcolor{red!20}-5.83\% & \cellcolor{red!20}-12.25\% & \cellcolor{yellow!20}0.00\% \\
    Yacht & \cellcolor{red!20}-1.24\% & \cellcolor{red!20}-2.69\% & \cellcolor{yellow!20}0.00\% \\
    \hline
    \end{tabular}
\end{table*}


==> tables/ablation_fe.tex <==
\begin{table*}[!th]
\centering
\caption{Performance gain (relative to the our basic \textsf{MFAN} model (PT-n/a)) with different designs on feature embedding (FE), self-attention (SA), aggregation functions (AGG), and pre-training (PT). Note that the basic \textsf{MFAN} is with missingness-aware addition for FE, column attention for SA, and the $\mathtt{[CLS]}$ embedding for AGG.}
\label{tab:ablation_all}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\hline
 & FE & FE & SA & SA & AGG & AGG & PT & PT & PT & PT \\ \hline
 & concat & FSE~\cite{grangier2010fse} & row att.~\cite{somepalli2021saint} & col+row att. & flatten & FC & n/a & RV & RM & RV+RM \\ \hline
Concrete & \cellcolor{green!20}0.45\% & \cellcolor{red!20}-27.50\% & \cellcolor{red!20}-4.99\% & \cellcolor{red!20}-2.32\% & \cellcolor{red!20}-7.27\% & \cellcolor{red!20}-10.55\% & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}0.19\% & \cellcolor{green!20}1.81\% & \cellcolor{green!20}0.31\% \\ \hline
Energy & \cellcolor{red!20}-31.58\% & \cellcolor{red!20}-183.08\% & \cellcolor{red!20}-6.42\% & \cellcolor{green!20}3.08\% & \cellcolor{red!20}-2.24\% & \cellcolor{green!20}3.58\% & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}17.39\% & \cellcolor{green!20}6.61\% & \cellcolor{green!20}15.10\% \\ \hline
Housing & \cellcolor{red!20}-6.50\% & \cellcolor{red!20}-75.20\% & \cellcolor{red!20}-4.07\% & \cellcolor{red!20}-9.23\% & \cellcolor{green!20}7.27\% & \cellcolor{green!20}1.21\% & \cellcolor{yellow!20}0.00\% & \cellcolor{red!20}-7.62\% & \cellcolor{red!20}-2.18\% & \cellcolor{green!20}4.94\% \\ \hline
Kin8nm & \cellcolor{green!20}0.88\% & \cellcolor{red!20}-31.19\% & \cellcolor{red!20}-19.19\% & \cellcolor{red!20}-16.78\% & \cellcolor{red!20}-6.78\% & \cellcolor{red!20}-7.93\% & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}10.57\% & \cellcolor{green!20}0.98\% & \cellcolor{green!20}12.49\% \\ \hline
Naval & \cellcolor{red!20}-16.51\% & \cellcolor{red!20}-47.16\% & \cellcolor{red!20}-27.70\% & \cellcolor{red!20}-48.74\% & \cellcolor{red!20}-139.86\% & \cellcolor{red!20}-53.79\% & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}20.57\% & \cellcolor{red!20}-1.70\% & \cellcolor{red!20}-1.99\% \\ \hline
Power & \cellcolor{red!20}-3.15\% & \cellcolor{red!20}-22.40\% & \cellcolor{green!20}1.58\% & \cellcolor{green!20}1.25\% & \cellcolor{green!20}1.98\% & \cellcolor{green!20}2.20\% & \cellcolor{yellow!20}0.00\% & \cellcolor{red!20}-0.69\% & \cellcolor{red!20}-0.29\% & \cellcolor{red!20}-0.42\% \\ \hline
Wine & \cellcolor{red!20}-0.60\% & \cellcolor{red!20}-10.66\% & \cellcolor{red!20}-19.78\% & \cellcolor{red!20}-17.35\% & \cellcolor{red!20}-5.83\% & \cellcolor{red!20}-12.25\% & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}10.19\% & \cellcolor{red!20}-0.01\% & \cellcolor{red!20}-0.98\% \\ \hline
Yacht & \cellcolor{green!20}10.50\% & \cellcolor{red!20}-104.99\% & \cellcolor{red!20}-14.89\% & \cellcolor{red!20}-5.92\% & \cellcolor{red!20}-1.24\% & \cellcolor{red!20}-2.69\% & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}0.13\% & \cellcolor{green!20}12.53\% & \cellcolor{green!20}10.58\% \\ \hline
\end{tabular}
}
\end{table*}

% \begin{table*}[htbp]
%     % \renewcommand{\arraystretch}{1.1}
%     \caption{Performance gain (relative to the \textit{join-complex} solution) with six different options for the design of the feature embedding layer.}
%     \label{tab:ablation_fe}
%     \centering
%     \begin{tabular}{l|c|c|c|c|c|c}
%     \hline
%      & part-basic & part-simple & part-complex & join-basic & join-simple & join-complex \\
%     \hline
%     Concrete & \cellcolor{red!20}-20.01\% & \cellcolor{red!20}-6.91\% & \cellcolor{green!20}0.45\% & \cellcolor{red!20}-27.50\% & \cellcolor{red!20}-18.16\% & \cellcolor{yellow!20}0.00\% \\
%     Energy & \cellcolor{red!20}-127.23\% & \cellcolor{red!20}-32.99\% & \cellcolor{red!20}-31.58\% & \cellcolor{red!20}-183.08\% & \cellcolor{red!20}-35.24\% & \cellcolor{yellow!20}0.00\% \\
%     Housing & \cellcolor{red!20}-8.03\% & \cellcolor{red!20}-49.21\% & \cellcolor{red!20}-6.50\% & \cellcolor{red!20}-75.20\% & \cellcolor{red!20}-31.51\% & \cellcolor{yellow!20}0.00\% \\
%     Kin8nm & \cellcolor{green!20}0.13\% & \cellcolor{red!20}-1.22\% & \cellcolor{green!20}0.88\% & \cellcolor{red!20}-31.19\% & \cellcolor{red!20}-1.18\% & \cellcolor{yellow!20}0.00\% \\
%     Naval & \cellcolor{red!20}-39.24\% & \cellcolor{red!20}-25.26\% & \cellcolor{red!20}-16.51\% & \cellcolor{red!20}-47.16\% & \cellcolor{red!20}-35.03\% & \cellcolor{yellow!20}0.00\% \\
%     Power & \cellcolor{red!20}-2.90\% & \cellcolor{red!20}-4.21\% & \cellcolor{red!20}-3.15\% & \cellcolor{red!20}-22.40\% & \cellcolor{red!20}-2.94\% & \cellcolor{yellow!20}0.00\% \\
%     Wine & \cellcolor{red!20}-3.12\% & \cellcolor{red!20}-1.20\% & \cellcolor{red!20}-0.60\% & \cellcolor{red!20}-10.66\% & \cellcolor{red!20}-6.46\% & \cellcolor{yellow!20}0.00\% \\
%     Yacht & \cellcolor{green!20}13.08\% & \cellcolor{green!20}14.97\% & \cellcolor{green!20}10.50\% & \cellcolor{red!20}-104.99\% & \cellcolor{green!20}3.41\% & \cellcolor{yellow!20}0.00\% \\
%     \hline
%     \end{tabular}
% \end{table*}


==> tables/ablation_mh.tex <==
\begin{table*}[htbp]
    % \renewcommand{\arraystretch}{1.1}
    \caption{Performance gain (relative to the normal self-attention version) with different layer designs of transformer encoder. The normal version containing only self-attention blocks is denoted as \textit{col}, and the modified version containing both intersample attention and self-attention blocks is denoted as \textit{col+row}. The number in brackets indicates the number of heads in the multi-head attention (default is 2).}
    \label{tab:ablation_mh}
    \centering
    \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.1\textwidth}|>{\centering\arraybackslash}p{0.1\textwidth}|>{\centering\arraybackslash}p{0.1\textwidth}}
    \hline
     & col (2) & col+row (2) & col+row (4) \\
    \hline
    Concrete & \cellcolor{yellow!20}0.00\% & \cellcolor{red!20}-4.99\% & \cellcolor{red!20}-2.32\% \\
    Energy & \cellcolor{yellow!20}0.00\% & \cellcolor{red!20}-6.42\% & \cellcolor{green!20}3.08\% \\
    Housing & \cellcolor{yellow!20}0.00\% & \cellcolor{red!20}-4.07\% & \cellcolor{red!20}-9.23\% \\
    Kin8nm & \cellcolor{yellow!20}0.00\% & \cellcolor{red!20}-19.19\% & \cellcolor{red!20}-16.78\% \\
    Naval & \cellcolor{yellow!20}0.00\% & \cellcolor{red!20}-27.70\% & \cellcolor{red!20}-48.74\% \\
    Power & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}1.58\% & \cellcolor{green!20}1.25\% \\
    Wine & \cellcolor{yellow!20}0.00\% & \cellcolor{red!20}-19.78\% & \cellcolor{red!20}-17.35\% \\
    Yacht & \cellcolor{yellow!20}0.00\% & \cellcolor{red!20}-14.89\% & \cellcolor{red!20}-5.92\% \\
    \hline
    \end{tabular}
\end{table*}


==> tables/ablation_pt.tex <==
\begin{table}[htbp]
    % \renewcommand{\arraystretch}{1.1}
    \caption{This table shows the performance gain (relative to no pre-training) with different choices of pre-training tasks. The "rx" denotes pre-training the model with feature value restoration task, the "rm" denotes pre-training with missing mask value restoration task, and the "rx+rm" denotes pre-training with both tasks.}
    \label{tab:ablation_pt}
    \centering
    \begin{tabular}{c|c|c|c|c}
    \hline
     & none & rx & rm & rx+rm \\
    \hline
    Concrete & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}0.19\% & \cellcolor{green!20}1.81\% & \cellcolor{green!20}0.31\% \\
    Energy & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}17.39\% & \cellcolor{green!20}6.61\% & \cellcolor{green!20}15.10\% \\
    Housing & \cellcolor{yellow!20}0.00\% & \cellcolor{red!20}-7.62\% & \cellcolor{red!20}-2.18\% & \cellcolor{green!20}4.94\% \\
    Kin8nm & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}10.57\% & \cellcolor{green!20}0.98\% & \cellcolor{green!20}12.49\% \\
    Naval & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}20.57\% & \cellcolor{red!20}-1.70\% & \cellcolor{red!20}-1.99\% \\
    Power & \cellcolor{yellow!20}0.00\% & \cellcolor{red!20}-0.69\% & \cellcolor{red!20}-0.29\% & \cellcolor{red!20}-0.42\% \\
    Wine & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}10.19\% & \cellcolor{red!20}-0.01\% & \cellcolor{red!20}-0.98\% \\
    Yacht & \cellcolor{yellow!20}0.00\% & \cellcolor{green!20}0.13\% & \cellcolor{green!20}12.53\% & \cellcolor{green!20}10.58\% \\
    \hline
    \end{tabular}
\end{table}


==> tables/datasets.tex <==
\begin{table}[!t]
    % \renewcommand{\arraystretch}{0.7}
    \caption{Dataset statistics. The number in the brackets indicates the number of class labels.}
    \label{tab:dataset}
    \centering
    % \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{l|r|r|c}
              & \# instances & \# features & task \\
    % \hline
    \hline
    Concrete  &        1,030 &           8 & regression \\
    Energy    &          768 &           8 & regression \\
    Housing   &          506 &          13 & regression \\
    Kin8nm    &        8,192 &           8 & regression \\
    Naval     &       11,934 &          17 & regression \\
    Power     &        9,568 &           4 & regression \\
    Wine      &        1,599 &          11 & regression \\
    Yacht     &          308 &           6 & regression \\
    \hline
    Avila     &       20,867 &          10 & classification (12) \\
    Eye       &       14,980 &          14 & classification (2) \\
    Letter    &       20,000 &          16 & classification (26) \\
    Pendigits &       10,092 &          16 & classification (10) \\
    Phishing  &       11,055 &          68 & classification (2) \\
    Segment   &        2,310 &          19 & classification (7) \\
    Spam      &        4,601 &          57 & classification (2) \\
    \end{tabular}
    % }
\end{table}


==> tables/overall_compare_cls.tex <==
\begin{table*}[!th]
    \caption{Mean F1 scores over 5 trials for the proposed model and competitors on classification datasets (with 0\% missing). }
    \label{tab:overall_cls_0}
    % \renewcommand{\arraystretch}{1.1}
    \centering
    % \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
    & Avila & Eye & Letter & Pendigits & Phishing & Segment & Spam \\
    \hline
    mean & 0.6952 $\pm$ 0.0116 & 0.8742 $\pm$ 0.0136 & \underline{0.8720 $\pm$ 0.0104} & \underline{0.9892 $\pm$ 0.0015} & \underline{0.9669 $\pm$ 0.0032} & \underline{0.9677 $\pm$ 0.0103} & \underline{0.9305 $\pm$ 0.0103} \\
    k-NN & 0.6686 $\pm$ 0.0102 & 0.8624 $\pm$ 0.0093 & 0.8302 $\pm$ 0.0196 & 0.9877 $\pm$ 0.0015 & 0.9653 $\pm$ 0.0015 & 0.9484 $\pm$ 0.0088 & 0.9252 $\pm$ 0.0079 \\
    MICE & 0.6686 $\pm$ 0.0102 & 0.8624 $\pm$ 0.0093 & 0.8302 $\pm$ 0.0196 & 0.9877 $\pm$ 0.0015 & 0.9653 $\pm$ 0.0015 & 0.9484 $\pm$ 0.0088 & 0.9252 $\pm$ 0.0079 \\
    GAIN & 0.6979 $\pm$ 0.0280 & 0.8768 $\pm$ 0.0131 & 0.8612 $\pm$ 0.0088 & 0.9880 $\pm$ 0.0016 & 0.9650 $\pm$ 0.0022 & 0.9618 $\pm$ 0.0115 & 0.9301 $\pm$ 0.0064 \\
    \hline
    D-Tree & 0.6063 $\pm$ 0.0029 & 0.6410 $\pm$ 0.0231 & 0.4379 $\pm$ 0.0131 & 0.8181 $\pm$ 0.0082 & 0.9171 $\pm$ 0.0060 & 0.9138 $\pm$ 0.0054 & 0.8699 $\pm$ 0.0079 \\
    GAIN(e) & \underline{0.7182 $\pm$ 0.0178} & \underline{0.8772 $\pm$ 0.0224} & 0.8680 $\pm$ 0.0150 & 0.9882 $\pm$ 0.0015 & 0.9659 $\pm$ 0.0040 & 0.9591 $\pm$ 0.0151 & 0.9281 $\pm$ 0.0030 \\
    GRAPE & 0.4351 $\pm$ 0.0788 & 0.4344 $\pm$ 0.2845 & 0.5031 $\pm$ 0.0820 & 0.9069 $\pm$ 0.0327 & 0.9387 $\pm$ 0.0188 & 0.9237 $\pm$ 0.0276 & 0.9189 $\pm$ 0.0079 \\
    \textsf{MFAN} & \textbf{0.9983 $\pm$ 0.0007} & \textbf{0.9774 $\pm$ 0.0046} & \textbf{0.9718 $\pm$ 0.0044} & \textbf{0.9955 $\pm$ 0.0011} & \textbf{0.9694 $\pm$ 0.0075} & \textbf{0.9731 $\pm$ 0.0081} & \textbf{0.9308 $\pm$ 0.0068} \\
    \hline
    % \end{tabular}
    % \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
    % \hline
    % & Pendigits & Phishing & Segment & Spam \\
    % \hline
    % mean & \underline{0.9892 $\pm$ 0.0015} & \underline{0.9669 $\pm$ 0.0032} & \underline{0.9677 $\pm$ 0.0103} & \underline{0.9305 $\pm$ 0.0103} \\
    % k-NN & 0.9877 $\pm$ 0.0015 & 0.9653 $\pm$ 0.0015 & 0.9484 $\pm$ 0.0088 & 0.9252 $\pm$ 0.0079 \\
    % MICE & 0.9877 $\pm$ 0.0015 & 0.9653 $\pm$ 0.0015 & 0.9484 $\pm$ 0.0088 & 0.9252 $\pm$ 0.0079 \\
    % GAIN & 0.9880 $\pm$ 0.0016 & 0.9650 $\pm$ 0.0022 & 0.9618 $\pm$ 0.0115 & 0.9301 $\pm$ 0.0064 \\
    % \hline
    % D-Tree & 0.8181 $\pm$ 0.0082 & 0.9171 $\pm$ 0.0060 & 0.9138 $\pm$ 0.0054 & 0.8699 $\pm$ 0.0079 \\
    % GAIN(e) & 0.9882 $\pm$ 0.0015 & 0.9659 $\pm$ 0.0040 & 0.9591 $\pm$ 0.0151 & 0.9281 $\pm$ 0.0030 \\
    % GRAPE & 0.9069 $\pm$ 0.0327 & 0.9387 $\pm$ 0.0188 & 0.9237 $\pm$ 0.0276 & 0.9189 $\pm$ 0.0079 \\
    % Ours & \textbf{0.9955 $\pm$ 0.0011} & \textbf{0.9694 $\pm$ 0.0075} & \textbf{0.9731 $\pm$ 0.0081} & \textbf{0.9308 $\pm$ 0.0068} \\
    % \hline
    \end{tabular}
    % }
\end{table*}

% \begin{table*}[htbp]
%     \renewcommand{\arraystretch}{1.1}
%     \caption{Mean F1 scores over 5 trials for the proposed model and competitors on classification datasets (with 10\% missing). We highlight the best result in bold and the second-best result in underline.}
%     \label{tab:overall_cls_1}
%     \centering
%     \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.256\textwidth}|>{\centering\arraybackslash}p{0.257\textwidth}|>{\centering\arraybackslash}p{0.256\textwidth}}
%     \hline
%     & Avila & Eye & Letter \\
%     \hline
%     mean & 0.6445 $\pm$ 0.0212 & 0.7768 $\pm$ 0.0096 & 0.7454 $\pm$ 0.0153 \\
%     k-NN & 0.6228 $\pm$ 0.0169 & \underline{0.8481 $\pm$ 0.0098} & \underline{0.8186 $\pm$ 0.0083} \\
%     MICE & 0.6134 $\pm$ 0.0196 & 0.8179 $\pm$ 0.0125 & 0.7531 $\pm$ 0.0069 \\
%     GAIN & 0.6450 $\pm$ 0.0166 & 0.7924 $\pm$ 0.0187 & 0.7468 $\pm$ 0.0106 \\
%     \hline
%     D-Tree & 0.5373 $\pm$ 0.0319 & 0.6347 $\pm$ 0.0146 & 0.3660 $\pm$ 0.0056 \\
%     GAIN(e) & \underline{0.6557 $\pm$ 0.0114} & 0.8157 $\pm$ 0.0175 & 0.7839 $\pm$ 0.0160 \\
%     GRAPE & 0.4608 $\pm$ 0.0442 & 0.5515 $\pm$ 0.1845 & 0.4375 $\pm$ 0.1444 \\
%     Ours & \textbf{0.8974 $\pm$ 0.0086} & \textbf{0.9309 $\pm$ 0.0078} & \textbf{0.9369 $\pm$ 0.0045} \\
%     \hline
%     \end{tabular}
%     \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
%     \hline
%     & Pendigits & Phishing & Segment & Spam \\
%     \hline
%     mean & 0.9597 $\pm$ 0.0060 & 0.9537 $\pm$ 0.0033 & 0.9117 $\pm$ 0.0060 & \textbf{0.9144 $\pm$ 0.0070} \\
%     k-NN & \underline{0.9837 $\pm$ 0.0025} & \textbf{0.9631 $\pm$ 0.0057} & \textbf{0.9455 $\pm$ 0.0058} & 0.9125 $\pm$ 0.0064 \\
%     MICE & 0.9772 $\pm$ 0.0039 & \underline{0.9618 $\pm$ 0.0034} & 0.9246 $\pm$ 0.0109 & 0.9106 $\pm$ 0.0078 \\
%     GAIN & 0.9573 $\pm$ 0.0040 & 0.9596 $\pm$ 0.0031 & 0.9206 $\pm$ 0.0146 & 0.9131 $\pm$ 0.0106 \\
%     \hline
%     D-Tree & 0.7847 $\pm$ 0.0112 & 0.9127 $\pm$ 0.0050 & 0.8854 $\pm$ 0.0136 & 0.8534 $\pm$ 0.0188 \\
%     GAIN(e) & 0.9665 $\pm$ 0.0035 & 0.9546 $\pm$ 0.0036 & 0.9326 $\pm$ 0.0118 & \underline{0.9135 $\pm$ 0.0094} \\
%     GRAPE & 0.8771 $\pm$ 0.0270 & 0.9391 $\pm$ 0.0082 & 0.8395 $\pm$ 0.1998 & 0.7511 $\pm$ 0.2792 \\
%     Ours & \textbf{0.9880 $\pm$ 0.0023} & 0.9444 $\pm$ 0.0111 & \underline{0.9408 $\pm$ 0.0094} & 0.9022 $\pm$ 0.0105 \\
%     \hline
%     \end{tabular}
% \end{table*}

\begin{table*}[!th]
    % \renewcommand{\arraystretch}{1.1}
    \caption{Mean F1 scores over 5 trials for the proposed model and competitors on classification datasets (with 20\% missing). }
    \label{tab:overall_cls_2}
    \centering
    % \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
    & Avila & Eye & Letter & Pendigits & Phishing & Segment & Spam \\
    \hline
    mean & 0.6052 $\pm$ 0.0150 & 0.7192 $\pm$ 0.0040 & 0.6461 $\pm$ 0.0103 & 0.9274 $\pm$ 0.0047 & 0.9459 $\pm$ 0.0041 & 0.8701 $\pm$ 0.0175 & \underline{0.8981 $\pm$ 0.0052} \\
    k-NN & 0.5876 $\pm$ 0.0144 & \underline{0.8024 $\pm$ 0.0135} & \underline{0.7745 $\pm$ 0.0118} & \underline{0.9695 $\pm$ 0.0044} & \textbf{0.9600 $\pm$ 0.0022} & \textbf{0.9420 $\pm$ 0.0114} & 0.8949 $\pm$ 0.0055 \\
    MICE & 0.5900 $\pm$ 0.0121 & 0.7551 $\pm$ 0.0215 & 0.6798 $\pm$ 0.0113 & 0.9577 $\pm$ 0.0019 & \underline{0.9572 $\pm$ 0.0026} & 0.9048 $\pm$ 0.0148 & 0.8943 $\pm$ 0.0082 \\
    GAIN & 0.5831 $\pm$ 0.0167 & 0.7284 $\pm$ 0.0200 & 0.6499 $\pm$ 0.0094 & 0.9208 $\pm$ 0.0051 & 0.9551 $\pm$ 0.0052 & 0.9066 $\pm$ 0.0143 & \textbf{0.9056 $\pm$ 0.0112} \\
    \hline
    D-Tree & 0.4603 $\pm$ 0.0082 & 0.5745 $\pm$ 0.0512 & 0.3188 $\pm$ 0.0079 & 0.7338 $\pm$ 0.0047 & 0.9064 $\pm$ 0.0050 & 0.8505 $\pm$ 0.0142 & 0.8266 $\pm$ 0.0125 \\
    GAIN(e) & \underline{0.6209 $\pm$ 0.0087} & 0.7686 $\pm$ 0.0235 & 0.7197 $\pm$ 0.0119 & 0.9470 $\pm$ 0.0042 & 0.9500 $\pm$ 0.0031 & 0.9043 $\pm$ 0.0073 & 0.8972 $\pm$ 0.0133 \\
    GRAPE & 0.4605 $\pm$ 0.0346 & 0.6203 $\pm$ 0.0072 & 0.3905 $\pm$ 0.0388 & 0.7886 $\pm$ 0.0714 & 0.9358 $\pm$ 0.0062 & 0.9063 $\pm$ 0.0218 & 0.8512 $\pm$ 0.1028 \\
    \textsf{MFAN} & \textbf{0.7827 $\pm$ 0.0042} & \textbf{0.8706 $\pm$ 0.0078} & \textbf{0.8837 $\pm$ 0.0064} & \textbf{0.9770 $\pm$ 0.0028} & 0.9379 $\pm$ 0.0034 & \underline{0.9162 $\pm$ 0.0117} & 0.8955 $\pm$ 0.0067 \\
    \hline
    % \end{tabular}
    % \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
    % \hline
    % & Pendigits & Phishing & Segment & Spam \\
    % \hline
    % mean & 0.9274 $\pm$ 0.0047 & 0.9459 $\pm$ 0.0041 & 0.8701 $\pm$ 0.0175 & \underline{0.8981 $\pm$ 0.0052} \\
    % k-NN & \underline{0.9695 $\pm$ 0.0044} & \textbf{0.9600 $\pm$ 0.0022} & \textbf{0.9420 $\pm$ 0.0114} & 0.8949 $\pm$ 0.0055 \\
    % MICE & 0.9577 $\pm$ 0.0019 & \underline{0.9572 $\pm$ 0.0026} & 0.9048 $\pm$ 0.0148 & 0.8943 $\pm$ 0.0082 \\
    % GAIN & 0.9208 $\pm$ 0.0051 & 0.9551 $\pm$ 0.0052 & 0.9066 $\pm$ 0.0143 & \textbf{0.9056 $\pm$ 0.0112} \\
    % \hline
    % D-Tree & 0.7338 $\pm$ 0.0047 & 0.9064 $\pm$ 0.0050 & 0.8505 $\pm$ 0.0142 & 0.8266 $\pm$ 0.0125 \\
    % GAIN(e) & 0.9470 $\pm$ 0.0042 & 0.9500 $\pm$ 0.0031 & 0.9043 $\pm$ 0.0073 & 0.8972 $\pm$ 0.0133 \\
    % GRAPE & 0.7886 $\pm$ 0.0714 & 0.9358 $\pm$ 0.0062 & 0.9063 $\pm$ 0.0218 & 0.8512 $\pm$ 0.1028 \\
    % Ours & \textbf{0.9770 $\pm$ 0.0028} & 0.9379 $\pm$ 0.0034 & \underline{0.9162 $\pm$ 0.0117} & 0.8955 $\pm$ 0.0067 \\
    % \hline
    \end{tabular}
    % }
\end{table*}

% \begin{table*}[htbp]
%     \renewcommand{\arraystretch}{1.1}
%     \caption{Mean F1 scores over 5 trials for the proposed model and competitors on classification datasets (with 30\% missing). We highlight the best result in bold and the second-best result in underline.}
%     \label{tab:overall_cls_3}
%     \centering
%     \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.256\textwidth}|>{\centering\arraybackslash}p{0.257\textwidth}|>{\centering\arraybackslash}p{0.256\textwidth}}
%     \hline
%     & Avila & Eye & Letter \\
%     \hline
%     mean & 0.5573 $\pm$ 0.0124 & 0.6793 $\pm$ 0.0085 & 0.5721 $\pm$ 0.0099 \\
%     k-NN & 0.5286 $\pm$ 0.0106 & 0.7085 $\pm$ 0.0123 & 0.6266 $\pm$ 0.0076 \\
%     MICE & 0.5224 $\pm$ 0.0044 & 0.6923 $\pm$ 0.0186 & 0.5902 $\pm$ 0.0045 \\
%     GAIN & 0.5519 $\pm$ 0.0114 & 0.6852 $\pm$ 0.0058 & 0.5695 $\pm$ 0.0057 \\
%     \hline
%     D-Tree & 0.4439 $\pm$ 0.0115 & 0.5874 $\pm$ 0.0322 & 0.2403 $\pm$ 0.0341 \\
%     GAIN(e) & \underline{0.5740 $\pm$ 0.0101} & \underline{0.7260 $\pm$ 0.0247} & \underline{0.6367 $\pm$ 0.0243} \\
%     GRAPE & 0.4447 $\pm$ 0.0226 & 0.6195 $\pm$ 0.0069 & 0.3518 $\pm$ 0.0442 \\
%     Ours & \textbf{0.6802 $\pm$ 0.0033} & \textbf{0.8161 $\pm$ 0.0068} & \textbf{0.8005 $\pm$ 0.0081} \\
%     \hline
%     \end{tabular}
%     \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
%     \hline
%     & Pendigits & Phishing & Segment & Spam \\
%     \hline
%     mean & 0.8814 $\pm$ 0.0035 & 0.9326 $\pm$ 0.0044 & 0.8259 $\pm$ 0.0255 & 0.8876 $\pm$ 0.0090 \\
%     k-NN & 0.9027 $\pm$ 0.0066 & \textbf{0.9471 $\pm$ 0.0020} & \textbf{0.8979 $\pm$ 0.0090} & 0.8780 $\pm$ 0.0102 \\
%     MICE & \underline{0.9249 $\pm$ 0.0045} & \underline{0.9451 $\pm$ 0.0027} & 0.8724 $\pm$ 0.0240 & 0.8779 $\pm$ 0.0061 \\
%     GAIN & 0.8819 $\pm$ 0.0097 & 0.9442 $\pm$ 0.0051 & 0.8637 $\pm$ 0.0261 & \underline{0.8905 $\pm$ 0.0089} \\
%     \hline
%     D-Tree & 0.6314 $\pm$ 0.0276 & 0.9030 $\pm$ 0.0071 & 0.8149 $\pm$ 0.0125 & 0.8146 $\pm$ 0.0054 \\
%     GAIN(e) & 0.9136 $\pm$ 0.0090 & 0.9334 $\pm$ 0.0036 & 0.8785 $\pm$ 0.0152 & \textbf{0.8938 $\pm$ 0.0086} \\
%     GRAPE & 0.7426 $\pm$ 0.0281 & 0.9269 $\pm$ 0.0059 & 0.8776 $\pm$ 0.0295 & 0.8638 $\pm$ 0.0794 \\
%     Ours & \textbf{0.9551 $\pm$ 0.0049} & 0.9273 $\pm$ 0.0014 & \underline{0.8819 $\pm$ 0.0074} & 0.8873 $\pm$ 0.0147 \\
%     \hline
%     \end{tabular}
% \end{table*}

% \begin{table*}[htbp]
%     \renewcommand{\arraystretch}{1.1}
%     \caption{Mean F1 scores over 5 trials for the proposed model and competitors on classification datasets (with 40\% missing). We highlight the best result in bold and the second-best result in underline.}
%     \label{tab:overall_cls_4}
%     \centering
%     \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.256\textwidth}|>{\centering\arraybackslash}p{0.257\textwidth}|>{\centering\arraybackslash}p{0.256\textwidth}}
%     \hline
%     & Avila & Eye & Letter \\
%     \hline
%     mean & 0.5232 $\pm$ 0.0152 & 0.6473 $\pm$ 0.0065 & 0.4849 $\pm$ 0.0125 \\
%     k-NN & 0.4885 $\pm$ 0.0226 & 0.6237 $\pm$ 0.0185 & 0.5142 $\pm$ 0.0056 \\
%     MICE & 0.4919 $\pm$ 0.0101 & 0.6734 $\pm$ 0.0159 & 0.5262 $\pm$ 0.0033 \\
%     GAIN & 0.5142 $\pm$ 0.0100 & 0.6569 $\pm$ 0.0026 & 0.4912 $\pm$ 0.0059 \\
%     \hline
%     D-Tree & 0.4209 $\pm$ 0.0111 & 0.5498 $\pm$ 0.0530 & 0.1220 $\pm$ 0.0231 \\
%     GAIN(e) & \underline{0.5410 $\pm$ 0.0105} & \underline{0.6869 $\pm$ 0.0034} & \underline{0.5466 $\pm$ 0.0190} \\
%     GRAPE & 0.4337 $\pm$ 0.0195 & 0.4331 $\pm$ 0.2836 & 0.2993 $\pm$ 0.0200 \\
%     Ours & \textbf{0.6074 $\pm$ 0.0070} & \textbf{0.7359 $\pm$ 0.0098} & \textbf{0.6975 $\pm$ 0.0162} \\
%     \hline
%     \end{tabular}
%     \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
%     \hline
%     & Pendigits & Phishing & Segment & Spam \\
%     \hline
%     mean & 0.8331 $\pm$ 0.0103 & 0.9191 $\pm$ 0.0032 & 0.7910 $\pm$ 0.0201 & \underline{0.8777 $\pm$ 0.0102} \\
%     k-NN & 0.7823 $\pm$ 0.0083 & 0.9265 $\pm$ 0.0100 & 0.8025 $\pm$ 0.0145 & 0.8566 $\pm$ 0.0083 \\
%     MICE & \underline{0.8812 $\pm$ 0.0081} & \textbf{0.9343 $\pm$ 0.0033} & 0.8203 $\pm$ 0.0259 & 0.8628 $\pm$ 0.0027 \\
%     GAIN & 0.8338 $\pm$ 0.0092 & \underline{0.9309 $\pm$ 0.0013} & 0.8243 $\pm$ 0.0230 & \textbf{0.8815 $\pm$ 0.0117} \\
%     \hline
%     D-Tree & 0.5006 $\pm$ 0.0019 & 0.8898 $\pm$ 0.0064 & 0.7666 $\pm$ 0.0188 & 0.7886 $\pm$ 0.0076 \\
%     GAIN(e) & 0.8769 $\pm$ 0.0033 & 0.9188 $\pm$ 0.0062 & \underline{0.8418 $\pm$ 0.0129} & 0.8768 $\pm$ 0.0088 \\
%     GRAPE & 0.6651 $\pm$ 0.0626 & 0.9174 $\pm$ 0.0091 & 0.8377 $\pm$ 0.0390 & 0.7956 $\pm$ 0.2655 \\
%     Ours & \textbf{0.9253 $\pm$ 0.0031} & 0.9126 $\pm$ 0.0079 & \textbf{0.8431 $\pm$ 0.0175} & 0.8692 $\pm$ 0.0130 \\
%     \hline
%     \end{tabular}
% \end{table*}

\begin{table*}[!th]
    % \renewcommand{\arraystretch}{1.1}
    \caption{Mean F1 scores over 5 trials for the proposed model and competitors on classification datasets (with 50\% missing). }
    \label{tab:overall_cls_5}
    \centering
    % \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
    & Avila & Eye & Letter & Pendigits & Phishing & Segment & Spam \\
    \hline
    mean & 0.4828 $\pm$ 0.0137 & 0.6269 $\pm$ 0.0073 & 0.4067 $\pm$ 0.0189 & 0.7658 $\pm$ 0.0096 & 0.9060 $\pm$ 0.0031 & 0.7253 $\pm$ 0.0246 & 0.8506 $\pm$ 0.0086 \\
    k-NN & 0.4496 $\pm$ 0.0172 & 0.5857 $\pm$ 0.0107 & 0.4022 $\pm$ 0.0067 & 0.7272 $\pm$ 0.0167 & 0.9100 $\pm$ 0.0044 & 0.6813 $\pm$ 0.0242 & 0.8259 $\pm$ 0.0160 \\
    MICE & 0.4342 $\pm$ 0.0203 & 0.6025 $\pm$ 0.0079 & 0.4419 $\pm$ 0.0085 & 0.8172 $\pm$ 0.0163 & \textbf{0.9149 $\pm$ 0.0047} & 0.7764 $\pm$ 0.0092 & 0.8496 $\pm$ 0.0173 \\
    GAIN & 0.4687 $\pm$ 0.0083 & 0.6262 $\pm$ 0.0100 & 0.4069 $\pm$ 0.0031 & 0.7684 $\pm$ 0.0070 & \underline{0.9129 $\pm$ 0.0018} & \underline{0.7852 $\pm$ 0.0249} & \underline{0.8557 $\pm$ 0.0137} \\
    \hline
    D-Tree & 0.3950 $\pm$ 0.0172 & 0.5151 $\pm$ 0.0486 & 0.0789 $\pm$ 0.0181 & 0.4219 $\pm$ 0.0111 & 0.8721 $\pm$ 0.0059 & 0.7146 $\pm$ 0.0193 & 0.7556 $\pm$ 0.0149 \\
    GAIN(e) & \underline{0.4970 $\pm$ 0.0091} & \underline{0.6580 $\pm$ 0.0097} & \underline{0.4724 $\pm$ 0.0183} & \underline{0.8175 $\pm$ 0.0100} & 0.8983 $\pm$ 0.0040 & 0.7808 $\pm$ 0.0236 & 0.8510 $\pm$ 0.0077 \\
    GRAPE & 0.4052 $\pm$ 0.0088 & 0.5524 $\pm$ 0.1845 & 0.2555 $\pm$ 0.0183 & 0.6373 $\pm$ 0.0610 & 0.9026 $\pm$ 0.0079 & 0.7778 $\pm$ 0.0400 & \textbf{0.8622 $\pm$ 0.0142} \\
    \textsf{MFAN} & \textbf{0.5342 $\pm$ 0.0121} & \textbf{0.6764 $\pm$ 0.0218} & \textbf{0.5741 $\pm$ 0.0117} & \textbf{0.8832 $\pm$ 0.0061} & 0.8957 $\pm$ 0.0051 & \textbf{0.8063 $\pm$ 0.0160} & 0.8448 $\pm$ 0.0151 \\
    \hline
    % \end{tabular}
    % \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
    % \hline
    % & Pendigits & Phishing & Segment & Spam \\
    % \hline
    % mean & 0.7658 $\pm$ 0.0096 & 0.9060 $\pm$ 0.0031 & 0.7253 $\pm$ 0.0246 & 0.8506 $\pm$ 0.0086 \\
    % k-NN & 0.7272 $\pm$ 0.0167 & 0.9100 $\pm$ 0.0044 & 0.6813 $\pm$ 0.0242 & 0.8259 $\pm$ 0.0160 \\
    % MICE & 0.8172 $\pm$ 0.0163 & \textbf{0.9149 $\pm$ 0.0047} & 0.7764 $\pm$ 0.0092 & 0.8496 $\pm$ 0.0173 \\
    % GAIN & 0.7684 $\pm$ 0.0070 & \underline{0.9129 $\pm$ 0.0018} & \underline{0.7852 $\pm$ 0.0249} & \underline{0.8557 $\pm$ 0.0137} \\
    % \hline
    % D-Tree & 0.4219 $\pm$ 0.0111 & 0.8721 $\pm$ 0.0059 & 0.7146 $\pm$ 0.0193 & 0.7556 $\pm$ 0.0149 \\
    % GAIN(e) & \underline{0.8175 $\pm$ 0.0100} & 0.8983 $\pm$ 0.0040 & 0.7808 $\pm$ 0.0236 & 0.8510 $\pm$ 0.0077 \\
    % GRAPE & 0.6373 $\pm$ 0.0610 & 0.9026 $\pm$ 0.0079 & 0.7778 $\pm$ 0.0400 & \textbf{0.8622 $\pm$ 0.0142} \\
    % Ours & \textbf{0.8832 $\pm$ 0.0061} & 0.8957 $\pm$ 0.0051 & \textbf{0.8063 $\pm$ 0.0160} & 0.8448 $\pm$ 0.0151 \\
    % \hline
    \end{tabular}
    % }
\end{table*}


==> tables/overall_compare_reg.tex <==
\begin{table*}[!th]
    % \tiny
    % \renewcommand{\arraystretch}{1.1}
    \caption{Mean RMSE scores for the proposed \textsf{MFAN} and competitors on regression task (with 0\% missing). We highlight the best result in bold and the second-best result in underline.}
    % \vspace{-5pt}
    \label{tab:overall_0}
    \centering
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \hline
    & Concrete & Energy & Housing & Kin8nm & Naval & Power & Wine & Yacht \\
    \hline
    mean & 11.2238 $\pm$ 0.5967 & 3.0954 $\pm$ 0.1583 & 5.4516 $\pm$ 0.4645 & 0.2023 $\pm$ 0.0017 & 0.0020 $\pm$ 0.0001 & 4.5209 $\pm$ 0.0633 & 0.6241 $\pm$ 0.0163 & 9.9055 $\pm$ 2.0482 \\
    k-NN & 10.8318 $\pm$ 0.6055 & 3.0911 $\pm$ 0.1572 & 5.1937 $\pm$ 0.5308 & 0.2024 $\pm$ 0.0015 & 0.0020 $\pm$ 0.0001 & 4.5172 $\pm$ 0.0682 & \underline{0.6238 $\pm$ 0.0157} & 9.8878 $\pm$ 2.0637 \\
    MICE & 10.8318 $\pm$ 0.6055 & 3.0911 $\pm$ 0.1572 & 5.1937 $\pm$ 0.5308 & 0.2024 $\pm$ 0.0015 & 0.0020 $\pm$ 0.0001 & 4.5172 $\pm$ 0.0682 & \underline{0.6238 $\pm$ 0.0157} & 9.8878 $\pm$ 2.0637 \\
    GAIN & 11.2291 $\pm$ 0.5960 & 3.2066 $\pm$ 0.2180 & 5.1308 $\pm$ 0.4138 & 0.2024 $\pm$ 0.0016 & \underline{0.0020 $\pm$ 0.0000} & 4.5178 $\pm$ 0.0677 & 0.6255 $\pm$ 0.0163 & 9.9004 $\pm$ 2.0948 \\
    \hline
    D-Tree & 9.4878 $\pm$ 0.3525 & 2.6530 $\pm$ 0.0498 & 4.7908 $\pm$ 0.5226 & 0.2168 $\pm$ 0.0031 & 0.0042 $\pm$ 0.0001 & 5.7864 $\pm$ 0.0430 & 0.6596 $\pm$ 0.0170 & \underline{2.1401 $\pm$ 0.0873} \\
    GAIN(e) & 11.2274 $\pm$ 0.5981 & 3.2055 $\pm$ 0.2160 & 5.2008 $\pm$ 0.5618 & 0.2023 $\pm$ 0.0016 & 0.0020 $\pm$ 0.0001 & 4.5187 $\pm$ 0.0661 & 0.6259 $\pm$ 0.0163 & 9.9006 $\pm$ 2.0877 \\
    GRAPE & \underline{6.6157 $\pm$ 3.1362} & \underline{0.6028 $\pm$ 0.1155} & \underline{4.2132 $\pm$ 0.6562} & \underline{0.0913 $\pm$ 0.0159} & 0.0075 $\pm$ 0.0001 & \underline{4.1172 $\pm$ 0.1311} & 0.7115 $\pm$ 0.0928 & 2.7826 $\pm$ 4.5529 \\
    \textsf{MFAN} & \textbf{5.1578 $\pm$ 0.4182} & \textbf{0.5183 $\pm$ 0.0332} & \textbf{3.6764 $\pm$ 0.9037} & \textbf{0.0755 $\pm$ 0.0021} & \textbf{0.0015 $\pm$ 0.0004} & \textbf{3.5946 $\pm$ 0.0440} & \textbf{0.6094 $\pm$ 0.0170} & \textbf{0.7494 $\pm$ 0.2959} \\
    \hline
    \end{tabular}
    }
    % \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
    % \hline
    % & Naval & Power & Wine & Yacht \\
    % \hline
    % mean & 0.0020 $\pm$ 0.0001 & 4.5209 $\pm$ 0.0633 & 0.6241 $\pm$ 0.0163 & 9.9055 $\pm$ 2.0482 \\
    % k-NN & 0.0020 $\pm$ 0.0001 & 4.5172 $\pm$ 0.0682 & \underline{0.6238 $\pm$ 0.0157} & 9.8878 $\pm$ 2.0637 \\
    % MICE & 0.0020 $\pm$ 0.0001 & 4.5172 $\pm$ 0.0682 & \underline{0.6238 $\pm$ 0.0157} & 9.8878 $\pm$ 2.0637 \\
    % GAIN & \underline{0.0020 $\pm$ 0.0000} & 4.5178 $\pm$ 0.0677 & 0.6255 $\pm$ 0.0163 & 9.9004 $\pm$ 2.0948 \\
    % \hline
    % D-Tree & 0.0042 $\pm$ 0.0001 & 5.7864 $\pm$ 0.0430 & 0.6596 $\pm$ 0.0170 & \underline{2.1401 $\pm$ 0.0873} \\
    % GAIN(e) & 0.0020 $\pm$ 0.0001 & 4.5187 $\pm$ 0.0661 & 0.6259 $\pm$ 0.0163 & 9.9006 $\pm$ 2.0877 \\
    % GRAPE & 0.0075 $\pm$ 0.0001 & \underline{4.1172 $\pm$ 0.1311} & 0.7115 $\pm$ 0.0928 & 2.7826 $\pm$ 4.5529 \\
    % Ours & \textbf{0.0015 $\pm$ 0.0004} & \textbf{3.5946 $\pm$ 0.0440} & \textbf{0.6094 $\pm$ 0.0170} & \textbf{0.7494 $\pm$ 0.2959} \\
    % \hline
    % \end{tabular}
\end{table*}

\begin{table*}[!th]
    % \renewcommand{\arraystretch}{1.1}
    \caption{Mean RMSE scores for the proposed \textsf{MFAN} and competitors on regression task (with 20\% missing).}
    % \vspace{-5pt}
    \label{tab:overall_1}
    \centering
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \hline
    & Concrete & Energy & Housing & Kin8nm & Naval & Power & Wine & Yacht \\
    \hline
    mean & 11.8420 $\pm$ 0.6463 & 3.8811 $\pm$ 0.1812 & 5.5567 $\pm$ 0.5067 & 0.2090 $\pm$ 0.0018 & 0.0075 $\pm$ 0.0001 & 6.2970 $\pm$ 0.0669 & 0.6373 $\pm$ 0.0208 & 10.2546 $\pm$ 1.9564 \\
    k-NN & 11.0813 $\pm$ 0.6900 & 3.2514 $\pm$ 0.1936 & 5.2031 $\pm$ 0.3619 & 0.2102 $\pm$ 0.0020 & \textbf{0.0023 $\pm$ 0.0001} & 5.6004 $\pm$ 0.0877 & \textbf{0.6317 $\pm$ 0.0162} & 10.2840 $\pm$ 1.9361 \\
    MICE & 11.1387 $\pm$ 0.6741 & 3.1773 $\pm$ 0.1792 & 5.3025 $\pm$ 0.4417 & 0.2089 $\pm$ 0.0021 & \underline{0.0032 $\pm$ 0.0001} & 5.1326 $\pm$ 0.1021 & \underline{0.6321 $\pm$ 0.0191} & 10.1952 $\pm$ 1.9795 \\
    GAIN & 11.8191 $\pm$ 0.6384 & 3.3836 $\pm$ 0.2210 & 5.1728 $\pm$ 0.3606 & 0.2092 $\pm$ 0.0017 & 0.0048 $\pm$ 0.0003 & 6.5645 $\pm$ 0.4863 & 0.6384 $\pm$ 0.0209 & 10.4109 $\pm$ 1.9208 \\
    \hline
    D-Tree & 9.9178 $\pm$ 0.4140 & 2.8880 $\pm$ 0.0858 & 4.7177 $\pm$ 0.6766 & 0.2297 $\pm$ 0.0046 & 0.0044 $\pm$ 0.0000 & 6.1726 $\pm$ 0.2009 & 0.6704 $\pm$ 0.0181 & \textbf{3.9736 $\pm$ 1.6463} \\
    GAIN(e) & 12.0342 $\pm$ 0.2055 & 3.4502 $\pm$ 0.3082 & 6.1810 $\pm$ 0.7387 & 0.2093 $\pm$ 0.0018 & 0.0049 $\pm$ 0.0004 & 5.1343 $\pm$ 0.1148 & 0.6403 $\pm$ 0.0208 & 11.6738 $\pm$ 1.7668 \\
    GRAPE & \textbf{7.9863 $\pm$ 0.5262} & \underline{1.6426 $\pm$ 0.4127} & \underline{4.3753 $\pm$ 0.5837} & \textbf{0.1446 $\pm$ 0.0051} & 0.0075 $\pm$ 0.0001 & \underline{4.7617 $\pm$ 0.1343} & 0.7430 $\pm$ 0.0630 & 5.1690 $\pm$ 2.0713 \\
    \textsf{MFAN} & \underline{8.2914 $\pm$ 0.4530} & \textbf{1.5988 $\pm$ 0.2160} & \textbf{4.3026 $\pm$ 0.5718} & \underline{0.1464 $\pm$ 0.0041} & 0.0063 $\pm$ 0.0014 & \textbf{4.6973 $\pm$ 0.1952} & 0.6409 $\pm$ 0.0142 & \underline{4.6242 $\pm$ 1.6281} \\
    \hline
    \end{tabular}
    }
    % \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
    % \hline
    % & Naval & Power & Wine & Yacht \\
    % \hline
    % mean & 0.0075 $\pm$ 0.0001 & 6.2970 $\pm$ 0.0669 & 0.6373 $\pm$ 0.0208 & 10.2546 $\pm$ 1.9564 \\
    % k-NN & \textbf{0.0023 $\pm$ 0.0001} & 5.6004 $\pm$ 0.0877 & \textbf{0.6317 $\pm$ 0.0162} & 10.2840 $\pm$ 1.9361 \\
    % MICE & \underline{0.0032 $\pm$ 0.0001} & 5.1326 $\pm$ 0.1021 & \underline{0.6321 $\pm$ 0.0191} & 10.1952 $\pm$ 1.9795 \\
    % GAIN & 0.0048 $\pm$ 0.0003 & 6.5645 $\pm$ 0.4863 & 0.6384 $\pm$ 0.0209 & 10.4109 $\pm$ 1.9208 \\
    % \hline
    % D-Tree & 0.0044 $\pm$ 0.0000 & 6.1726 $\pm$ 0.2009 & 0.6704 $\pm$ 0.0181 & \textbf{3.9736 $\pm$ 1.6463} \\
    % GAIN(e) & 0.0049 $\pm$ 0.0004 & 5.1343 $\pm$ 0.1148 & 0.6403 $\pm$ 0.0208 & 11.6738 $\pm$ 1.7668 \\
    % GRAPE & 0.0075 $\pm$ 0.0001 & \underline{4.7617 $\pm$ 0.1343} & 0.7430 $\pm$ 0.0630 & 5.1690 $\pm$ 2.0713 \\
    % Ours & 0.0063 $\pm$ 0.0014 & \textbf{4.6973 $\pm$ 0.1952} & 0.6409 $\pm$ 0.0142 & \underline{4.6242 $\pm$ 1.6281} \\
    % \hline
    % \end{tabular}
\end{table*}

% \begin{table*}[htbp]
%     \renewcommand{\arraystretch}{1.1}
%     \caption{Mean RMSE scores over 5 trials for the proposed model and competitors on regression datasets (with 20\% missing). We highlight the best result in bold and the second-best result in underline.}
%     \label{tab:overall_2}
%     \centering
%     \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
%     \hline
%     & Concrete & Energy & Housing & Kin8nm \\
%     \hline
%     mean & 12.5537 $\pm$ 0.7188 & 4.4987 $\pm$ 0.2119 & 5.7922 $\pm$ 0.4122 & 0.2164 $\pm$ 0.0016 \\
%     k-NN & 11.8921 $\pm$ 0.4337 & 3.5232 $\pm$ 0.2053 & 5.5660 $\pm$ 0.5190 & 0.2202 $\pm$ 0.0015 \\
%     MICE & 11.7056 $\pm$ 0.6890 & 3.4967 $\pm$ 0.2187 & 5.6505 $\pm$ 0.4899 & 0.2165 $\pm$ 0.0013 \\
%     GAIN & 12.5465 $\pm$ 0.7173 & 3.7271 $\pm$ 0.3167 & 5.8724 $\pm$ 0.4177 & 0.2170 $\pm$ 0.0015 \\
%     \hline
%     D-Tree & 11.0912 $\pm$ 0.4140 & 3.1755 $\pm$ 0.1305 & 5.4682 $\pm$ 0.4790 & 0.2366 $\pm$ 0.0023 \\
%     GAIN(e) & 12.8952 $\pm$ 0.7164 & 3.8342 $\pm$ 0.4028 & 6.9527 $\pm$ 0.7002 & 0.2163 $\pm$ 0.0018 \\
%     GRAPE & \textbf{9.5582 $\pm$ 0.5855} & \underline{2.2741 $\pm$ 0.4072} & \textbf{4.6656 $\pm$ 0.5321} & \textbf{0.1809 $\pm$ 0.0045} \\
%     Ours & \underline{9.8218 $\pm$ 0.5438} & \textbf{2.0857 $\pm$ 0.3727} & \underline{5.0357 $\pm$ 0.7572} & \underline{0.1833 $\pm$ 0.0038} \\
%     \hline
%     \end{tabular}
%     \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
%     \hline
%     & Naval & Power & Wine & Yacht \\
%     \hline
%     mean & 0.0075 $\pm$ 0.0001 & 7.4590 $\pm$ 0.1061 & 0.6437 $\pm$ 0.0188 & 11.0047 $\pm$ 1.7229 \\
%     k-NN & \textbf{0.0029 $\pm$ 0.0003} & 6.6445 $\pm$ 0.0896 & \textbf{0.6351 $\pm$ 0.0191} & 11.1333 $\pm$ 1.6232 \\
%     MICE & \underline{0.0044 $\pm$ 0.0001} & 5.8899 $\pm$ 0.0637 & \underline{0.6381 $\pm$ 0.0177} & 10.9230 $\pm$ 1.7168 \\
%     GAIN & 0.0057 $\pm$ 0.0004 & 7.2338 $\pm$ 0.1685 & 0.6471 $\pm$ 0.0179 & 11.2312 $\pm$ 1.6204 \\
%     \hline
%     D-Tree & 0.0053 $\pm$ 0.0002 & 7.5038 $\pm$ 0.2335 & 0.6871 $\pm$ 0.0247 & \textbf{6.3338 $\pm$ 1.9654} \\
%     GAIN(e) & 0.0059 $\pm$ 0.0006 & 5.8041 $\pm$ 0.0515 & 0.6528 $\pm$ 0.0175 & 12.0067 $\pm$ 1.7962 \\
%     GRAPE & 0.0075 $\pm$ 0.0001 & \underline{5.5905 $\pm$ 0.1299} & 0.7320 $\pm$ 0.0629 & 7.6052 $\pm$ 2.1520 \\
%     Ours & 0.0059 $\pm$ 0.0020 & \textbf{5.4837 $\pm$ 0.0700} & 0.6522 $\pm$ 0.0150 & \underline{7.2028 $\pm$ 2.0819} \\
%     \hline
%     \end{tabular}
% \end{table*}

% \begin{table*}[htbp]
%     \renewcommand{\arraystretch}{1.1}
%     \caption{Mean RMSE scores over 5 trials for the proposed model and competitors on regression datasets (with 30\% missing). We highlight the best result in bold and the second-best result in underline.}
%     \label{tab:overall_3}
%     \centering
%     \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
%     \hline
%     & Concrete & Energy & Housing & Kin8nm \\
%     \hline
%     mean & 13.1440 $\pm$ 0.8080 & 4.9662 $\pm$ 0.2933 & 6.2301 $\pm$ 0.4714 & 0.2228 $\pm$ 0.0014 \\
%     k-NN & 12.4452 $\pm$ 0.7876 & 4.1590 $\pm$ 0.4066 & 5.8782 $\pm$ 0.5901 & 0.2292 $\pm$ 0.0018 \\
%     MICE & 12.4207 $\pm$ 0.6433 & 3.8817 $\pm$ 0.2884 & 6.2939 $\pm$ 0.5288 & 0.2229 $\pm$ 0.0013 \\
%     GAIN & 13.1730 $\pm$ 0.8423 & 4.2569 $\pm$ 0.3965 & 6.0143 $\pm$ 0.5207 & 0.2232 $\pm$ 0.0014 \\
%     \hline
%     D-Tree & 12.3381 $\pm$ 0.6397 & 3.5519 $\pm$ 0.3357 & 5.7651 $\pm$ 0.6005 & 0.2421 $\pm$ 0.0026 \\
%     GAIN(e) & 13.8241 $\pm$ 1.9598 & 4.3906 $\pm$ 0.2491 & 7.6757 $\pm$ 0.5200 & 0.2232 $\pm$ 0.0013 \\
%     GRAPE & \underline{10.8890 $\pm$ 0.5458} & \textbf{2.7928 $\pm$ 0.5017} & \textbf{5.0116 $\pm$ 0.6395} & \textbf{0.2038 $\pm$ 0.0033} \\
%     Ours & \textbf{10.8079 $\pm$ 0.9064} & \underline{2.8401 $\pm$ 0.2396} & \underline{5.6571 $\pm$ 0.6123} & \underline{0.2057 $\pm$ 0.0021} \\
%     \hline
%     \end{tabular}
%     \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
%     \hline
%     & Naval & Power & Wine & Yacht \\
%     \hline
%     mean & 0.0075 $\pm$ 0.0001 & 8.5127 $\pm$ 0.1195 & 0.6581 $\pm$ 0.0164 & 11.3346 $\pm$ 1.5441 \\
%     k-NN & 0.0068 $\pm$ 0.0001 & 7.9056 $\pm$ 0.1387 & \underline{0.6541 $\pm$ 0.0159} & 11.5874 $\pm$ 1.4306 \\
%     MICE & \textbf{0.0055 $\pm$ 0.0000} & \underline{7.2857 $\pm$ 0.1343} & \textbf{0.6479 $\pm$ 0.0143} & 11.5202 $\pm$ 1.5982 \\
%     GAIN & 0.0063 $\pm$ 0.0003 & 8.7412 $\pm$ 0.5451 & 0.6599 $\pm$ 0.0174 & 11.4752 $\pm$ 1.5136 \\
%     \hline
%     D-Tree & \underline{0.0057 $\pm$ 0.0001} & 8.7057 $\pm$ 0.3531 & 0.6989 $\pm$ 0.0232 & \textbf{7.5523 $\pm$ 1.1375} \\
%     GAIN(e) & 0.0065 $\pm$ 0.0003 & 7.5230 $\pm$ 0.2003 & 0.6731 $\pm$ 0.0214 & 11.9305 $\pm$ 1.7256 \\
%     GRAPE & 0.0075 $\pm$ 0.0001 & 7.5789 $\pm$ 3.0627 & 0.7715 $\pm$ 0.0687 & 9.7414 $\pm$ 2.2520 \\
%     Ours & 0.0076 $\pm$ 0.0001 & \textbf{6.4495 $\pm$ 0.1674} & 0.6789 $\pm$ 0.0225 & \underline{8.3819 $\pm$ 1.4812} \\
%     \hline
%     \end{tabular}
% \end{table*}

% \begin{table*}[htbp]
%     \renewcommand{\arraystretch}{1.1}
%     \caption{Mean RMSE scores over 5 trials for the proposed model and competitors on regression datasets (with 40\% missing). We highlight the best result in bold and the second-best result in underline.}
%     \label{tab:overall_4}
%     \centering
%     \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
%     \hline
%     & Concrete & Energy & Housing & Kin8nm \\
%     \hline
%     mean & 13.7707 $\pm$ 0.7379 & 5.4004 $\pm$ 0.4396 & 6.4594 $\pm$ 0.3287 & 0.2286 $\pm$ 0.0016 \\
%     k-NN & 13.2227 $\pm$ 0.7449 & 4.7182 $\pm$ 0.3327 & 6.2539 $\pm$ 0.2832 & 0.2351 $\pm$ 0.0011 \\
%     MICE & 12.9661 $\pm$ 0.7401 & 4.4003 $\pm$ 0.4621 & 6.3320 $\pm$ 0.5014 & 0.2290 $\pm$ 0.0017 \\
%     GAIN & 13.9811 $\pm$ 0.6833 & 4.8405 $\pm$ 0.3828 & 6.5075 $\pm$ 0.5132 & 0.2294 $\pm$ 0.0012 \\
%     \hline
%     D-Tree & 13.0605 $\pm$ 0.5631 & 4.0937 $\pm$ 0.5195 & 6.3414 $\pm$ 0.4305 & 0.2459 $\pm$ 0.0019 \\
%     GAIN(e) & 14.1038 $\pm$ 1.7840 & 4.6487 $\pm$ 0.2334 & 7.5536 $\pm$ 0.1746 & 0.2298 $\pm$ 0.0022 \\
%     GRAPE & \underline{12.0429 $\pm$ 0.4830} & \textbf{3.2680 $\pm$ 0.5959} & \textbf{5.8716 $\pm$ 1.2030} & \textbf{0.2197 $\pm$ 0.0029} \\
%     Ours & \textbf{11.6698 $\pm$ 0.6132} & \underline{3.5945 $\pm$ 0.3401} & \underline{5.9516 $\pm$ 0.5902} & \underline{0.2205 $\pm$ 0.0013} \\
%     \hline
%     \end{tabular}
%     \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
%     \hline
%     & Naval & Power & Wine & Yacht \\
%     \hline
%     mean & 0.0075 $\pm$ 0.0001 & 9.5473 $\pm$ 0.1438 & \underline{0.6758 $\pm$ 0.0227} & 11.9576 $\pm$ 1.4018 \\
%     k-NN & 0.0074 $\pm$ 0.0001 & 9.0384 $\pm$ 0.1710 & 0.6819 $\pm$ 0.0173 & 12.2772 $\pm$ 1.2155 \\
%     MICE & \underline{0.0063 $\pm$ 0.0000} & 9.0767 $\pm$ 0.1781 & \textbf{0.6626 $\pm$ 0.0145} & 12.3226 $\pm$ 1.4787 \\
%     GAIN & 0.0069 $\pm$ 0.0004 & 10.0054 $\pm$ 0.3771 & 0.6811 $\pm$ 0.0163 & 12.4256 $\pm$ 1.2711 \\
%     \hline
%     D-Tree & \textbf{0.0061 $\pm$ 0.0001} & 10.2309 $\pm$ 0.2120 & 0.7057 $\pm$ 0.0157 & \textbf{9.8115 $\pm$ 1.4552} \\
%     GAIN(e) & 0.0069 $\pm$ 0.0002 & 10.0019 $\pm$ 1.2133 & 0.6879 $\pm$ 0.0303 & 13.2579 $\pm$ 1.3314 \\
%     GRAPE & 0.0075 $\pm$ 0.0001 & \underline{8.6425 $\pm$ 2.6791} & 0.7914 $\pm$ 0.0678 & 10.7070 $\pm$ 1.9594 \\
%     Ours & 0.0076 $\pm$ 0.0001 & \textbf{7.6455 $\pm$ 0.0727} & 0.6969 $\pm$ 0.0178 & \underline{10.6758 $\pm$ 1.4915} \\
%     \hline
%     \end{tabular}
% \end{table*}

\begin{table*}[!tp]
    % \renewcommand{\arraystretch}{1.1}
    \caption{Mean RMSE scores for the proposed \textsf{MFAN} and competitors on regression task (with 50\% missing).}
    % \vspace{-5pt}
    \label{tab:overall_5}
    \centering
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \hline
    & Concrete & Energy & Housing & Kin8nm & Naval & Power & Wine & Yacht \\
    \hline
    mean & 14.4285 $\pm$ 0.8940 & 5.9777 $\pm$ 0.3822 & 6.8637 $\pm$ 0.2810 & 0.2352 $\pm$ 0.0024 & 0.0075 $\pm$ 0.0001 & 10.5848 $\pm$ 0.1459 & \underline{0.6908 $\pm$ 0.0279} & 12.6678 $\pm$ 1.2986 \\
    k-NN & 13.9109 $\pm$ 0.9808 & 5.5727 $\pm$ 0.3501 & 6.8623 $\pm$ 0.3617 & 0.2400 $\pm$ 0.0020 & 0.0075 $\pm$ 0.0001 & 10.2257 $\pm$ 0.1202 & 0.6973 $\pm$ 0.0195 & 13.0666 $\pm$ 1.0070 \\
    MICE & 13.6970 $\pm$ 1.0419 & 5.2829 $\pm$ 0.3703 & 6.7405 $\pm$ 0.3016 & 0.2437 $\pm$ 0.0054 & \underline{0.0069 $\pm$ 0.0001} & 10.5340 $\pm$ 0.1486 & \textbf{0.6836 $\pm$ 0.0182} & 12.8526 $\pm$ 1.0926 \\
    GAIN & 14.6027 $\pm$ 0.8428 & 5.5880 $\pm$ 0.5535 & 6.8838 $\pm$ 0.1991 & 0.2364 $\pm$ 0.0023 & 0.0073 $\pm$ 0.0001 & 11.5183 $\pm$ 0.4626 & 0.6953 $\pm$ 0.0248 & 13.0607 $\pm$ 1.4217 \\
    \hline
    D-Tree & \underline{13.0795 $\pm$ 0.3255} & 5.1186 $\pm$ 0.2344 & 6.8279 $\pm$ 0.8565 & 0.2488 $\pm$ 0.0017 & \textbf{0.0063 $\pm$ 0.0001} & 11.1129 $\pm$ 0.4797 & 0.7286 $\pm$ 0.0238 & \textbf{11.2330 $\pm$ 1.5221} \\
    GAIN(e) & 14.8297 $\pm$ 1.6707 & 5.0129 $\pm$ 0.2556 & 7.6737 $\pm$ 0.5090 & 0.2368 $\pm$ 0.0031 & 0.0073 $\pm$ 0.0001 & 12.9210 $\pm$ 1.1353 & 0.7713 $\pm$ 0.0557 & 13.9553 $\pm$ 1.4363 \\
    GRAPE & 13.1634 $\pm$ 0.6244 & \underline{4.5120 $\pm$ 0.4871} & \textbf{5.9083 $\pm$ 0.8312} & \underline{0.2337 $\pm$ 0.0039} & 0.0075 $\pm$ 0.0001 & \underline{9.8123 $\pm$ 2.3099} & 0.7730 $\pm$ 0.0649 & 12.5659 $\pm$ 1.7555 \\
    \textsf{MFAN} & \textbf{12.7495 $\pm$ 0.7900} & \textbf{4.3555 $\pm$ 0.3137} & \underline{6.3877 $\pm$ 0.6323} & \textbf{0.2314 $\pm$ 0.0036} & 0.0073 $\pm$ 0.0007 & \textbf{9.0340 $\pm$ 0.0955} & 0.7260 $\pm$ 0.0223 & \underline{12.0166 $\pm$ 1.4094} \\
    \hline
    % \end{tabular}
    % \begin{tabular}{p{0.1\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}|>{\centering\arraybackslash}p{0.185\textwidth}}
    % \hline
    % & Naval & Power & Wine & Yacht \\
    % \hline
    % mean & 0.0075 $\pm$ 0.0001 & 10.5848 $\pm$ 0.1459 & \underline{0.6908 $\pm$ 0.0279} & 12.6678 $\pm$ 1.2986 \\
    % k-NN & 0.0075 $\pm$ 0.0001 & 10.2257 $\pm$ 0.1202 & 0.6973 $\pm$ 0.0195 & 13.0666 $\pm$ 1.0070 \\
    % MICE & \underline{0.0069 $\pm$ 0.0001} & 10.5340 $\pm$ 0.1486 & \textbf{0.6836 $\pm$ 0.0182} & 12.8526 $\pm$ 1.0926 \\
    % GAIN & 0.0073 $\pm$ 0.0001 & 11.5183 $\pm$ 0.4626 & 0.6953 $\pm$ 0.0248 & 13.0607 $\pm$ 1.4217 \\
    % \hline
    % D-Tree & \textbf{0.0063 $\pm$ 0.0001} & 11.1129 $\pm$ 0.4797 & 0.7286 $\pm$ 0.0238 & \textbf{11.2330 $\pm$ 1.5221} \\
    % GAIN(e) & 0.0073 $\pm$ 0.0001 & 12.9210 $\pm$ 1.1353 & 0.7713 $\pm$ 0.0557 & 13.9553 $\pm$ 1.4363 \\
    % GRAPE & 0.0075 $\pm$ 0.0001 & \underline{9.8123 $\pm$ 2.3099} & 0.7730 $\pm$ 0.0649 & 12.5659 $\pm$ 1.7555 \\
    % Ours & 0.0073 $\pm$ 0.0007 & \textbf{9.0340 $\pm$ 0.0955} & 0.7260 $\pm$ 0.0223 & \underline{12.0166 $\pm$ 1.4094} \\
    % \hline
    \end{tabular}
    }
\end{table*}


==> tables/overall_rank.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{table*}[!t]
\centering
\caption{Average rank over datasets on two tasks. }
\label{tab:rank_reg_cls}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{c|cccccc|cccccc}
\hline
\multicolumn{1}{l}{} & \multicolumn{6}{|c}{Regression} & \multicolumn{6}{|c}{Classification} \\ \hline
Missing \% & 0\% & 10\% & 20\% & 30\% & 40\% & 50\% & 0\% & 10\% & 20\% & 30\% & 40\% & 50\% \\ \hline
mean & 6.125 & 6.000 & 5.875 & 5.375 & 5.125 & 5.250 & \underline{2.571} & 4.714 & 4.857 & 5.000 & 4.571 & 4.286 \\
k-NN & 4.125 & 4.250 & 4.250 & 5.000 & 4.750 & 5.250 & 4.857 & \textbf{2.429} & \underline{2.571} & 3.143 & 5.286 & 5.857 \\
MICE & 4.000 & 3.625 & 3.750 & 3.625 & 3.500 & 3.875 & 4.857 & 3.857 & 4.000 & 4.143 & 3.429 & 4.000 \\
GAIN & 5.375 & 5.500 & 5.750 & 5.500 & 5.875 & 5.750 & 3.714 & 4.286 & 4.143 & 4.429 & 3.429 & 3.143 \\ \hline
D-Tree & 5.125 & 4.250 & 4.500 & 4.250 & 4.625 & 4.000 & 7.714 & 7.429 & 8.000 & 8.000 & 7.857 & 7.857 \\
GAIN(e) & 5.750 & 6.375 & 6.000 & 6.000 & 6.125 & 6.250 & 3.000 & 3.143 & 3.571 & \underline{2.429} & \underline{2.714} & \underline{2.857} \\
GRAPE & \underline{3.625} & \underline{3.375} & \underline{3.250} & \underline{3.250} & \textbf{3.000} & \underline{3.375} & 7.286 & 7.571 & 6.571 & 6.571 & 6.429 & 5.429 \\
\textsf{MFAN} & \textbf{1.000} & \textbf{2.625} & \textbf{2.625} & \textbf{3.000} & \textbf{3.000} & \textbf{2.125} & \textbf{1.000} & \underline{2.571} & \textbf{2.286} & \textbf{2.286} & \textbf{2.286} & \textbf{2.571} \\ \hline
\end{tabular}
}
\end{table*}

% \begin{table*}[!t]
%     % \renewcommand{\arraystretch}{1.1}
%     \caption{Average rank of each methods on regression datasets. }
%     \label{tab:rank_reg}
%     \centering
%     % \resizebox{\textwidth}{!}{
%     \begin{tabular}{c|c|c|c|c|c|c}
%     \hline
%     Missing Rate & 0\% & 10\% & 20\% & 30\% & 40\% & 50\% \\
%     \hline
%     mean & 6.125 & 6.000 & 5.875 & 5.375 & 5.125 & 5.250 \\
%     k-NN & 4.125 & 4.250 & 4.250 & 5.000 & 4.750 & 5.250 \\
%     MICE & 4.000 & 3.625 & 3.750 & 3.625 & 3.500 & 3.875 \\
%     GAIN & 5.375 & 5.500 & 5.750 & 5.500 & 5.875 & 5.750 \\
%     \hline
%     D-Tree & 5.125 & 4.250 & 4.500 & 4.250 & 4.625 & 4.000 \\
%     GAIN(e) & 5.750 & 6.375 & 6.000 & 6.000 & 6.125 & 6.250 \\
%     GRAPE & \underline{3.625} & \underline{3.375} & \underline{3.250} & \underline{3.250} & \textbf{3.000} & \underline{3.375} \\
%     Ours & \textbf{1.000} & \textbf{2.625} & \textbf{2.625} & \textbf{3.000} & \textbf{3.000} & \textbf{2.125} \\
%     \hline
%     \end{tabular}
%     % }
% \end{table*}

% \begin{table*}[htbp]
%     % \renewcommand{\arraystretch}{1.1}
%     \caption{Average rank of each methods on classification datasets.}
%     \label{tab:rank_cls}
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
%     \hline
%     Missing Rate & 0\% & 10\% & 20\% & 30\% & 40\% & 50\% \\
%     \hline
%     mean & \underline{2.571} & 4.714 & 4.857 & 5.000 & 4.571 & 4.286 \\
%     k-NN & 4.857 & \textbf{2.429} & \underline{2.571} & 3.143 & 5.286 & 5.857 \\
%     MICE & 4.857 & 3.857 & 4.000 & 4.143 & 3.429 & 4.000 \\
%     GAIN & 3.714 & 4.286 & 4.143 & 4.429 & 3.429 & 3.143 \\
%     \hline
%     D-Tree & 7.714 & 7.429 & 8.000 & 8.000 & 7.857 & 7.857 \\
%     GAIN(e) & 3.000 & 3.143 & 3.571 & \underline{2.429} & \underline{2.714} & \underline{2.857} \\
%     GRAPE & 7.286 & 7.571 & 6.571 & 6.571 & 6.429 & 5.429 \\
%     Ours & \textbf{1.000} & \underline{2.571} & \textbf{2.286} & \textbf{2.286} & \textbf{2.286} & \textbf{2.571} \\
%     \hline
%     \end{tabular}
% \end{table*}

% \begin{table*}[htbp]
%     \renewcommand{\arraystretch}{1.1}
%     \caption{Average rank of each methods on all datasets. We highlight the best result in bold and the second best result in underline.}
%     \label{tab:rank_all}
%     \centering
%     \begin{tabular}{p{0.14\textwidth}|>{\centering\arraybackslash}p{0.1\textwidth}|>{\centering\arraybackslash}p{0.1\textwidth}|>{\centering\arraybackslash}p{0.1\textwidth}|>{\centering\arraybackslash}p{0.1\textwidth}|>{\centering\arraybackslash}p{0.1\textwidth}|>{\centering\arraybackslash}p{0.1\textwidth}}
%     \hline
%     Missing Rate & 0\% & 10\% & 20\% & 30\% & 40\% & 50\% \\
%     \hline
%     mean & 4.467 & 5.400 & 5.400 & 5.200 & 4.867 & 4.800 \\
%     k-NN & 4.467 & \underline{3.400} & \underline{3.467} & 4.133 & 5.000 & 5.533 \\
%     MICE & \underline{4.400} & 3.733 & 3.867 & \underline{3.867} & \underline{3.467} & \underline{3.933} \\
%     GAIN & 4.600 & 4.933 & 5.000 & 5.000 & 4.733 & 4.533 \\
%     \hline
%     D-Tree & 6.333 & 5.733 & 6.133 & 6.000 & 6.133 & 5.800 \\
%     GAIN(e) & 4.467 & 4.867 & 4.867 & 4.333 & 4.533 & 4.667 \\
%     GRAPE & 5.333 & 5.333 & 4.800 & 4.800 & 4.600 & 4.333 \\
%     Ours & \textbf{1.000} & \textbf{2.600} & \textbf{2.467} & \textbf{2.667} & \textbf{2.667} & \textbf{2.333} \\
%     \hline
%     \end{tabular}
% \end{table*}

